Adapted variable density subsampling for compressed sensing

Recent results in compressed sensing showed that the optimal subsampling strategy should take into account the sparsity pattern of the signal at hand. This oracle-like knowledge, even though desirable, nevertheless remains elusive in most practical application. We try to close this gap by showing how the sparsity patterns can instead be characterised via a probability distribution on the supports of the sparse signals allowing us to again derive optimal subsampling strategies. This probability distribution can be easily estimated from signals of the same signal class, achieving state of the art performance in numerical experiments. Our approach also extends to structured acquisition, where instead of isolated measurements, blocks of measurements are taken.

==> sec_discussion.tex <==
%%%%%%%%%%%%%%%
% !TEX root = omp_perturbed.tex
%%%%%%%%%%%%%%
\section{Discussion}\label{sec:discussion}
%%%%%%%%%%%%%%
The above results showed that the optimal variable density subsampling strategy should not only depend on the structure of the sensing and sparsity matrices, but also on the distribution of sparsity patterns of the signals to be measured. We derived lower bounds on the number of measurements to ensure recovery of the sparse signals with high probability and derived a simple formula for the optimal subsampling strategy. We showed that this distribution can be estimated from a training set and that the resulting adapted subsampling scheme provides state of the art performance in a range of situations. For future work it would be interesting to analyse different settings of blocks of measurements, where explicit lower bounds on the number of measurements can be derived.
